Neural L1 Adaptive Control of Vehicle Lateral Dynamics

We address the problem of stable and robust control of vehicles with lateral error dynamics for the application of lane keeping. Lane departure is the primary reason for half of the fatalities in road accidents, making the development of stable, adaptive and robust controllers a necessity. Traditional linear feedback controllers achieve satisfactory tracking performance, however, they exhibit unstable behavior when uncertainties are induced into the system. Any disturbance or uncertainty introduced to the steering-angle input can be catastrophic for the vehicle. Therefore, controllers must be developed to actively handle such uncertainties. In this work, we introduce a Neural L1 Adaptive controller (Neural-L1) which learns the uncertainties in the lateral error dynamics of a front-steered Ackermann vehicle and guarantees stability and robustness. Our contributions are threefold: i) We extend the theoretical results for guaranteed stability and robustness of conventional L1 Adaptive controllers to Neural-L1; ii) We implement a Neural-L1 for the lane keeping application which learns uncertainties in the dynamics accurately; iii)We evaluate the performance of Neural-L1 on a physics-based simulator, PyBullet, and conduct extensive real-world experiments with the F1TENTH platform to demonstrate superior reference trajectory tracking performance of Neural-L1 compared to other state-of-the-art controllers, in the presence of uncertainties. Our project page, including supplementary material and videos, can be found at https://mukhe027.github.io/Neural-Adaptive-Control/

==> 3-background.tex <==
\section{Background}\label{Background}


==> 5-system_overview.tex <==
\section{System Overview}\label{System Overview}
In this section, we present the \emph{stability} theory for the \neural~after augmenting it with the DNN framework, to learn the uncertainties as adaptive laws. The complete \neural~architecture is shown in Fig.\ref{fig:adaptive_framework}. 
% with the traditional $\mathcal{L}_1$ adaptive control architecture from \cite{hovakimyan20111} shown in the red region and the augmented DNN framework from \cite{joshi2019deep} shown in the green region.
\begin{figure}[!htb]
\centering
% \subfloat{\includegraphics[width = 0.8\linewidth]
\subfloat{\includegraphics[width=0.5\textwidth]{fig/sim result plots/l1_adap_framework.pdf}}
\caption{Overview of our approach depicts the \ladap \cite{hovakimyan20111}  (red region), the neural network-based adaptive laws (green region) and the neural network training mechanism (blue region), adopted from \cite{joshi2019deep}.  }
\vspace{-10pt}
\label{fig:adaptive_framework}
\end{figure}
The stability analysis of \neural~consists of the following steps. First, we will define an ideal closed-loop reference system $\dot{x}_{ref}(t)$  with control law $u_{ref}(t)$. We will then use the $\mathcal{L}_1$ norm condition to show that $x_{ref}(t)$ is uniformly bounded in Lemma \ref{lem:l1_cond}. Next, we will analyse the transient and steady state performance of our controller by first defining the error dynamics as $\dot{\Tilde{x}}$, then presenting results of uniform boundedness of $\Tilde{x}(t)$ and convergence $\underset{t\rightarrow \infty}{\lim} \Tilde{x} =0$ in Lemma \ref{lem:pred_er} and Lemma \ref{lem:conv}, respectively. Finally, we provide the \emph{main} convergence results in Theorem~\ref{thrm:1} proving $x(t)$ converges to $x_{ref}(t)$ and $u(t)$ converges to $u_{ref}(t)$. We conclude this section providing the proof for Lyapunov stability of the complete controller after the augmentation of the DNN framework.    

\subsection{$\mathcal{L}_1$ Adaptive Control (\ladap) Architecture}
Consider the \emph{total} adaptive control law $u(t)$, consisting of linear feedback component, $u_m(t)$, and the adaptive control component $u_{ad}(t)$
\begin{align}\label{eq:totl_contrl_law}
    u(t) = u_m (t) + u_{ad}(t), ~ u_m(t) = - k_m x(t)
\end{align}
where $k_m \in \mathbb{R}^n$ renders $A_m  \triangleq A-B_1k_m$ Hurwitz, while $u_{ad}(t)$ is the adaptive component, to be defined shortly. The static feedback gain $k_m$, with the control law in \eqref{eq:totl_contrl_law} substituted in \eqref{eq:er_gnrl_st_sp}, leads to the following closed-loop system:
\begin{align} \label{eq:er_unct}
\dot{x}(t) &= A_mx(t) + B_1(u_{ad}(t)+ \Delta(x) + \Bar{\Delta}(x)) + B_2\dot{\Psi}_{des},\nonumber\\ 
 x(0) &= x_o; \quad y(t) =  c^T x(t) 
\end{align}
where $\Bar{\Delta}(x)) = \zeta^T x(t)$, which follows the relation from traditional \textit{adaptive controller} derivation. We refer the reader to \cite{slotine1991applied} for background reading on the theory of State Predictor-based MRAC as it forms the basis of derivation for the theory of \ladap.
Consequently, for a linearly parameterized system in \eqref{eq:er_unct}, we consider the state predictor as
\begin{align} \label{eq:st_prdctr}
\dot{\hat{x}}(t) &= A_m\hat{x}(t) + B_1(\hat{\Delta}(x(t))+\hat{\Bar{\Delta}}(x)+ u_{ad}(t)) + \scriptstyle B_2\dot{\Psi}_{des},\nonumber\\ ~\hat{x}(0) &= x_o; \quad y(t) =  c^T x(t) 
\end{align}
where $\hat{x}(t)\in \mathbb{R}^n$ is the state of the predictor and $\hat{\Delta}(x), \hat{\Bar{\Delta}}(x)= \hat{\zeta}x(t) \in \mathbb{R}^n$ are the estimates of the \textit{unknown} parameter $\Delta(x(t))\in \mathbb{R}^n$, and $\Bar{\Delta}(x)\in \mathbb{R}^n$.

The \emph{total} true uncertainty $(\Delta(x) + \Bar{\Delta}(x))$ is unknown\footnote{Note that dependence on time will only be shown when introducing new concepts or symbols. Subsequent usage will drop these dependencies for clarity of presentation.}, but it is assumed to be continuous over the compact set $D_x  \subset \mathbb{R}^n$. In this paper, we use the \emph{adaptive laws} from the traditional \ladap~to learn part of the total true uncertainty, $\Bar{\Delta}(x)$, and we use the augmented DNN framework to learn the \emph{residual} uncertainty, $\Delta(x)$. We use a DNN framework to represent a function when the basis vector is unknown. Using DNNs, a non-linearly parameterized network estimate of the uncertainty can be written as $\hat{\Delta}(x) \triangleq \theta_n^T \Phi(x)$, where $\theta_n \in \mathbb{R}^{k\times m}$ are network weights for the final layer and $\Phi(x)= \phi_n (\theta_{n-1}, \phi_{n-1}(\theta_{n-2},\phi_{n-2}(\dots))))$, is a $k$ dimensional feature vector which is a function of the inner layer weights, activations and inputs. The basis vector $\Phi(x)\in F:\mathbb{R}^n \rightarrow \mathbb{R}^k$ is considered to be Lipschitz continuous to ensure the existence and uniqueness of the solution. 

\subsection{Adaptive Control Law}
We now derive $u_{ad}$ in \eqref{eq:totl_contrl_law}. We know that the form of $u_m$ satisfies the matching conditions such that $A_m\triangleq A - B_1k_m$, which is a typical form of the \textit{full state feedback controller}. Further, we would like to choose $u_{ad}$ such that it cancels out $\Delta(x) + \Bar{\Delta}(x)$, however, since $\Delta(x)$ and $\Bar{\Delta}(x)$ are unknown, we \emph{estimate} $u_{ad}=\hat{\Delta}(x)+ \hat{\Bar{\Delta}}(x)$. 

From \cite{hovakimyan20111}, we know that \ladap~framework is implemented using a low-pass filter of the form $C(s)$, where $C(s)$ is a Bounded Input, Bounded Output (BIBO)-stable and stricly proper transfer function with DC gain $C(0)=1$, and its state space realization assumes zero initialization. Therefore, the control law term $u_{ad}$ is given by
\begin{align}\label{eq:u_ad_tf}
    u_{ad} (s)=- C(s)(\hat{\eta}(s) + \hat{\Bar{\eta}}(s)- k_g r(s)) 
\end{align}
where $r(s)$, $\hat{\eta}(s)$, $\hat{\Bar{\eta}}(s)$ are the Laplace transforms of reference signal $r(t)$, $\hat{\eta}(t) \triangleq  \hat{\Delta}(x(t))  $, and $\hat{\Bar{\eta}}(t) \triangleq  \hat{\Bar{\Delta}}(x(t))  $ , and the reference signal gain $k_g \triangleq -1/(c^T A_m^{-1}B_1)$.






In this paper, we are also using an \emph{online} DNN framework similar to \cite{joshi2019deep} to estimate \emph{residual} uncertainty, where the true estimates of the labeled pairs of state and true residual uncertainty $\{x(t),\Delta(x(t))\}$ are needed. 
% Since, the true uncertainty $\Delta(x(t))$ is unknown, we use generative networks to generate the estimates of the true uncertainty $\Delta(x(t))$, as done in \cite{joshi2019deep}. 
% Further, for online estimation of the parameter, we apply Deep-Model Reference Generative Network (D-MRGeN) from \cite{joshi2019deep}.
% The generative model estimate is denoted by $\Delta '(x)$ in the total control law of the system. 
To achieve the asymptotic convergence of the predictive model tracking error to zero, we substitute the DNN estimate in the controller $u_{ad}$, where 
\begin{align}
    \Delta'(x) = W^T \phi_n (\theta_{n-1}, \phi_{n-1}(\theta_{n-2},\phi_{n-2}(\dots))))
\end{align}

We now state Assumption 1 from \cite{joshi2019deep}.
 \begin{assumption} from \cite{joshi2019deep}\label{asum:1}
 Appealing to the universal approximation of neural networks we have that, for every given basis functions $\Phi(x)\in \mathcal{F}$ there exists unique ideal weights $W^* \in \mathbb{R}^{k\times m}$ and $\epsilon_1(x)\mathbb{R}^m$ such that the following approximation holds
 \end{assumption}
 \begin{align}
     \Delta(x) = W^{*^T} \Phi(x) +\epsilon_1(x), ~ \forall x \in D_x \subset \mathbb{R}^n
 \end{align}
 \begin{fact} from \cite{joshi2019deep}\label{fct:1}
 The network approximation error $\epsilon_1(x)$ is upper bounded, s.t. $\epsilon_1 = \sup_{x\in D_x}\|\epsilon_1(x)\|$, and can be made arbitrarily small given sufficiently large number of basis functions. 
 \end{fact}
 
 Next, we discuss the estimation method of the unknown true network parameters $W^*$. The unknown true network parameters $W^*$ are estimated using the estimation or the adaptive law given as
 \begin{align}\label{eq:adap_law1}
\dot{W}(x) = \Gamma_1 proj (W,\Tilde{x}^T(t)PB_1\Phi(x)),~ W(0) = W_0 \in D_x
\end{align}
where $\Tilde{x}\triangleq \hat{x}-x$ is the prediction error, $\Gamma_1 \in \mathbb{R}_+$ is the adaptation gain, and $P=P^T>0$ solves the algebraic Lyapunov equation $A_m^T P + P A_m= -Q$ for arbitrary symmetric $Q=Q^T>0$. The projection is confined to the set $D_x$. With the neural network-based \emph{adaptive law} stated in \eqref{eq:adap_law1}, the adaptation law from a \ladap~can be represented as
 \begin{align}\label{eq:adap_law2}
\dot{\hat{\zeta}}(x) = \Gamma_2 proj (\hat{\zeta},\Tilde{x}^T(t)PB_1x(t)),~ \hat{\zeta}(0) = \hat{\zeta}_0 \in D_x
\end{align}


Then, taking the Laplace transform of $u_{ad}(t)$, the adaptive control signal looks like
\begin{align}\label{eq:u_ad_tf1}
     u_{ad} (s)=- C(s)(\hat{\eta}(s) + \hat{\Bar{\eta}}(s)- k_g r(s)) 
\end{align}

Now that the \ladap~is defined using the relationships in \eqref{eq:totl_contrl_law}, \eqref{eq:st_prdctr}, \eqref{eq:u_ad_tf} and \eqref{eq:adap_law1}, with $k_m$ and $C(s)$, it must satisfy the $\mathcal{L}_1$-norm condition given by
\begin{align}\label{eq:l1norm}
    \lambda_1 \triangleq \|G(s) \|_{\mathcal{L}_1} L_1 < 1
\end{align}
where
$G(s) \triangleq H(s)(1-C(s)$, $H(s)\triangleq (s\mathbb{I}-A_m)^{-1}B_1$, $L_1\triangleq  \underset{\zeta\in D_x}{\max} \|\zeta\|_1$. However, in this work, since we are using neural networks to learn the \textit{residual} uncertainty parameter, we have an additional $\mathcal{L}_1$ norm condition to satisfy $\lambda_2 \triangleq \|G(s) \|_{\mathcal{L}_1} L_2 < 1$, where $L_2\triangleq  \underset{W\in D_x}{\max} \|W\|_1$.

Therefore, we define the following nonadaptive version of the adaptive control system, also known as  the closed-loop reference system of the class of systems in \eqref{eq:er_gnrl_st_sp}
\begin{align} \label{eq:closd_ref}
\dot{x}_{ref}(t) &=  B_1(u_{ref}(t)+ \Delta(x_{ref}(t))+ \bar{\zeta}^Tx_{ref}(t)) \dots \nonumber \\
&+ Ax_{ref}(t) + B_2\dot{\Psi}_{des}, ~~ x_{ref}(0) =x_0 \nonumber \\
 u_{ref} (s)=- &C(s)(\hat{\eta}(s) + \bar{\zeta}^Tx_{ref}(s)- k_g r(s)- k_m x_{ref}(s)) 
\end{align}


Next, we provide the first theoretical result in Lemma \ref{lem:l1_cond} where we signify the importance of the $\mathcal{L}_1$ condition, such that $x_{ref}(t)$ can be shown to be uniformly bounded.
\begin{lemma}\label{lem:l1_cond}
If $\|G(s)\|_{\mathcal{L}_1}L<1$, then the system in \eqref{eq:closd_ref} is bounded-input bounded-state stable with respect to the reference signal $r(t)$ and $x_0$.
\end{lemma}
\begin{proof}
From the definition of the closed-loop reference system in \eqref{eq:closd_ref} , it follows

\begin{align}
        x_{ref}(s) &= G(s)\eta(s) + G(s)\bar{\zeta}^Tx_{ref}(s) + k_g H(s)C(s)r(s)  \nonumber\\
        &\cdots+ H_1(s) f(s)+ x_{in}(s)
\end{align}
where $x_{in}(s) \triangleq (s\mathbb{I}-A_m)^{-1}x_o$, $\eta(s)$ is the Laplace transform of $\Delta(x_{ref}(t))$. Recalling the fact that $H(s),C(s)$ and $G(s)$ are proper BIBO-stable transfer functions, it follows from \eqref{eq:closd_ref} that for $\tau \in [0,\infty)$, the following bounds hold:
% \begin{align}
%    &\|x_{ref_{\tau}}\|_{\mathcal{L}_{\infty}} \leq \|G(s)\|_{\mathcal{L}_{1}}\|\eta_{\tau}\|_{\mathcal{L}_{\infty}} + \|G(s)\bar{\zeta}^T\|_{\mathcal{L}_1}\|x_{ref_{\tau}}\|_{\mathcal{L}_{\infty}}   \nonumber\\
%         &+ \|k_g H(s)C(s)\|_{\mathcal{L}_{1}}\|r_{\tau}\|_{\mathcal{L}_{\infty}}+ \|H_1(s) f(s)\|_{\mathcal{L}_{1}}+ \|x_{in_{\tau}} \|_{\mathcal{L}_{\infty}}
% \end{align}
% Since $A_m$ is Hurwitz, $x_{in}(t)$ is uniformly bounded. Thus, using the relation in \eqref{eq:l1norm} we can imply that
% \begin{align}\label{eq:bound_1}
% \|G(s) \zeta^T\|_{\mathcal{L}_1} = \max_{i=1,\dots, n}\|G_i(s)\|_{\mathcal{L}_1}\sum^n_{j=1}|\zeta_j |\leq \scriptstyle \|G(s) \|_{\mathcal{L}_1}  L_1<1
% \end{align}
% Consequently,
\begin{align}\label{eq:stabil}
   &\|x_{ref_{\tau}}\|_{\mathcal{L}_{\infty}} \leq \frac{\|G(s)\|_{\mathcal{L}_{1}}\|\eta_{\tau}\|_{\mathcal{L}_{\infty}}}{1-\|G(s)\bar{\zeta}^T\|_{\mathcal{L}_1}} + \frac{\|H_1(s) f(s)\|_{\mathcal{L}_{1}}}{1-\|G(s)\bar{\zeta}^T\|_{\mathcal{L}_1}} \cdots \nonumber\\
        &+ \frac{\|k_g H(s)C(s)\|_{\mathcal{L}_{1}}}{1-\|G(s)\bar{\zeta}^T\|_{\mathcal{L}_1}}\|r_{\tau}\|_{\mathcal{L}_{\infty}}+ \frac{\|x_{in_{\tau}} \|_{\mathcal{L}_{\infty}}}{1-\|G(s)\bar{\zeta}^T\|_{\mathcal{L}_1}}
\end{align}
Since $r(t)$ and $x_{in}(t)$ are uniformly bounded, and \eqref{eq:stabil} holds uniformly for $\tau \in [0,\infty)$, $x_{ref}(t)$ is uniformly bounded. This completes the proof. Note that the \textit{true uncertainty} $\Delta(x_{ref}(t))$ is assumed to be continuous and bounded over a compact domain $D_x \subset \mathbb{R}^n$, which implies $\eta(s)$ is also bounded.
\end{proof}



\subsection{Transient and Steady-State Performance}
For the error $\Tilde{x}=\hat{x}-x$, the error dynamics $\dot{\Tilde{x}}$, using \eqref{eq:er_unct} and \eqref{eq:st_prdctr} can be written as
\begin{align}\label{eq:er_dyn}
    \dot{\Tilde{x}} = A_m \Tilde{x} + B_1( \Tilde{W}^T \Phi(x) + \Tilde{\Bar{\zeta}}x(t))+ \epsilon_1(x)
    \end{align}
    where $\Tilde{W}\triangleq W^* -W$. Further, we let $\Tilde{\eta}(t) \triangleq \Tilde{W}^T\Phi(x(t))$, with $\Tilde{n}(s)$ being its Laplace transform and $\Tilde{\Bar{\eta}}(t) \triangleq \Tilde{\Bar{\zeta}}(t)x(t)$ with $\Tilde{\Bar{\eta}}(s)$ being its Laplace transform. Therefore, the error dynamics in frequency domain can be re-written as 
    \begin{align}\label{eq:er_dyn_fs}
    \Tilde{x}(s) = H(s)(\Tilde{\eta}(s) + \Tilde{\Bar{\eta}}(s) + \epsilon_1(x(s)))
    \end{align}
    where $\epsilon_1(x(s))$ is the Laplace transform of $\epsilon_1(x(t))$.
    Before we present the uniform boundedness result of $\Tilde{x}$ in Lemma \ref{lem:pred_er}, we state Assumption \ref{asum:2}
    \begin{assumption} from \cite{joshi2019deep}\label{asum:2}
    For uncertainty parameterized by unknown true weights $W^* \in \mathbb{R}^{k\times n}$ and known nonlinear $\phi(x)$, the ideal weight matrix is assumed to be upper bounded s.t. $\|W^*\|\leq W_b$.
    \end{assumption}
    
    \begin{lemma}\label{lem:pred_er}
    The prediction error $\Tilde{x}$  is uniformly bounded.
    \end{lemma}
    \begin{proof}
%    The feature vectors belong to a function class
% characterized by the inner layer network weights $\theta_i$ s.t $\Phi \in \mathcal{F}$. 
% Using the same manipulation process in Theorem~1 in \cite{joshi2019deep}, we will prove the Lyapunov stability under the assumption that inner layer of DNN presents us a feature which results in the worst possible approximation error compared to network with features before switch. 
For this purpose, we will denote $\Phi(x)$ as feature before switch and $\Bar{\Phi}(x)$ as the feature after switch. We define the error $\epsilon_2(x)$ as
\begin{align}
    \epsilon_2 (x) = \underset{\Bar{\Phi}\in F}{\sup} |W^T\Bar{\phi}(x) - W^T\Phi (x)|
\end{align}
Using Fact~\ref{fct:1}, we can upper bound $\epsilon_2(x)$ as $\Bar{\epsilon}_2=\underset{x\in D_x}{\sup} \|\epsilon_2 (x)\|$. Thus, by adding and subtracting the term $W^T \Bar{\Phi}(x)$, we can rewrite the error dynamics \eqref{eq:er_dyn}
\begin{align}\label{eq:er_dyn2}
    \dot{\Tilde{x}} &= A_m \Tilde{x} + B_1( W^{*T}\Phi (x) - W^T \Phi(x) +  W^T \Bar{\Phi}(x) \cdots \nonumber\\
    &- W^T \Bar{\Phi}(x)+ \Tilde{\Bar{\zeta}}x(t))+ \epsilon_1(x)
    \end{align}
    Then by applying Assumption~\ref{asum:1}, there exists $W^* \forall \Phi \in \mathcal{F}$ such that we can replace $W^{*T}\Phi(x)$ by $W^{*T}\Bar{\Phi}(x)$ in \eqref{eq:er_dyn} to obtain
    \begin{align}\label{eq:er_dyn3}
    \dot{\Tilde{x}} = A_m \Tilde{x} + B_1( \Tilde{W}^{*T}\Bar{\Phi} (x) + \Tilde{\Bar{\zeta}}x(t))+ \epsilon_1(x) + \epsilon_2 (x)
    \end{align}


Thus, we consider the following Lyapunov function
    
    \begin{align}\label{eq:lyapunov_1}
    V(\Tilde{x},\Tilde{W},\Tilde{\Bar{\zeta}}) = \Tilde{x}^T P \Tilde{x} + \frac{\Tilde{W}^T \Gamma_1^{-1}\Tilde{W}}{2} + \frac{\Tilde{\Bar{\zeta}}^T \Tilde{\Bar{\zeta}}}{\Gamma_2}
    \end{align}
   Now taking the time derivative of the Lyapunov function in \eqref{eq:lyapunov_1}, we get $\dot{V}$ as
     \begin{align}\label{eq:der_lyapunov_1}
    \dot{V}(\Tilde{x},\Tilde{W},\Tilde{\Bar{\zeta}}) \leq -\Tilde{x}^T Q \Tilde{x} + 2\Tilde{x}^T P \epsilon(x)
    \end{align}
    where $\epsilon(x) = \epsilon_1(x) + \epsilon_2 (x)$ and $\bar{\epsilon} = \Bar{\epsilon_1} + \Bar{\epsilon_2}$.
    Hence, Lyapunov stability $\dot{V}(\Tilde{x},\Tilde{W},\Tilde{\Bar{\zeta}})\leq0$ is obtained outside compact neighborhood of the origin $\Tilde{x}=0$, for some sufficiently large $\lambda_{\min}(Q)$ where we can show a lower bound on $\Tilde{x}$ as
    \begin{align}\label{eq:er_low_bnd}
      \|\Tilde{x}(t)\|\geq \frac{2 \lambda_{\max}(P)\Bar{\epsilon}}{\lambda_{\min}(Q)}  
    \end{align}
    Now, to show that $\Tilde{x}(t)$ is bounded, we know that $\Tilde{x}(t)$ is uniformly bounded. Next, since $\Tilde{x}(0)=0$ and in the vicinity of the compact neighborhood of the origin $\Tilde{x}(t)=0$, it follows that
    \begin{align}
        \lambda_{\min}(P) \|\Tilde{x}(t) \|^2 &\leq V(t) \leq V(0) =  \frac{\Tilde{W}(0)^T \Gamma_1^{-1}\Tilde{W}(0)}{2} \cdots \nonumber\\
        &+ \frac{\Tilde{\Bar{\zeta}}^T(x(0)) \Tilde{\Bar{\zeta}}(x(0))}{\Gamma_2}
    \end{align}
    The projection operators\footnote{Definition of projection operators can be found in \cite{hovakimyan20111}.} with Assumption \ref{asum:2} ensure that the error parameters $\Tilde{W}$ and $\Tilde{\bar{\zeta}}$ are bounded 
    % and so we have
    % \begin{align}
    % \frac{\Tilde{W}(0)^T \Gamma_1^{-1}\Tilde{W}(0)}{2} \leq \frac{4 \underset{W\in D_x}{\max}\|W\|^2}{\Gamma_1}, \cdots \nonumber \\
    % \frac{\Tilde{\Bar{\zeta}}^T(x(0)) \Tilde{\Bar{\zeta}}(x(0))}{\Gamma_2} \leq \frac{4 \underset{\zeta\in D_x}{\max}\|\zeta\|^2}{\Gamma_2}
    % \end{align}
    which leads to the following upper bound:
    % \begin{align}\label{eq:newprdt_tf}
    %     \|\Tilde{x}\|^2\leq \frac{W_{\max}}{\lambda_{\min}(P)\Gamma_1} + \frac{\zeta_{\max}}{\lambda_{\min}(P)\Gamma_2}
    % \end{align}
    % Since $\|\cdot\|_{\infty}\leq \|\cdot\|$, and this bound is uniform, the bound above yields
     \begin{align}\label{eq:bound}
        \|\Tilde{x}_{\tau}\|_{\mathcal{L}_{\infty}}\leq \sqrt{ \frac{W_{\max}}{\lambda_{\min}(P)\Gamma_1} + \frac{\zeta_{\max}}{\lambda_{\min}(P)\Gamma_2}}
    \end{align}
    which holds for every $\tau\geq 0$
    
    \end{proof}
    
    % Notice that the bounds on $\Tilde{x}$ are obtained independent of the control term $u_{ad}$. This implies that both $x$ and $\hat{x}$ can diverge at the same rate, maintaining a uniformly bounded error between the two. 
    % Further, the result in Lemma \ref{lem:conv} will prove that using the control law $u_{ad}$, the state of the predictor remains bounded and consequently leads to asymptotic convergence of the tracking error $\Tilde{x}$ to zero.
    Lemma~\ref{lem:conv} below proves for asymptotic convergence of the tracking error $\Tilde{x}$ to zero.
    \begin{lemma}\label{lem:conv}
    For adaptive control law given by $u_{ad}$ and if the condition in \eqref{eq:l1norm} holds, then we have the asymptotic convergence $\underset{t\rightarrow \infty}{\lim} \Tilde{x} =0$.
    \end{lemma}
    \begin{proof}
    For asymptotic convergence of $\Tilde{x}(t)$ to zero, we show $\hat{x}(t)$ with $u_{ad}(t)$ is uniformly bounded
    % Therefore, we have
    % \begin{align}
    %     \hat{x}(s) &= G(s)\hat{\eta}(s) + G(s)\hat{\bar{\eta}}(s) + k_g H(s)C(s)r(s) \cdots \nonumber\\
    %     &+ H_1(s) f(s)+ x_{in}(s)
    % \end{align}
    % where $H_1(s) \triangleq (s\mathbb{I} - A_m)^{-1} B_2$ and $f(s)= \mathcal{L}(\dot{\Psi}_{des})$ is the Laplace transform, 
    which leads to the following upper bound
    \begin{align}\label{eq:prdict_tf}
        &\|\hat{x}_{\tau}\|_{\mathcal{L}_{\infty}} = \|G(s)\|_{\mathcal{L}_{1}}\|\hat{\eta}_{\tau}\|_{\mathcal{L}_{\infty}} + \|G(s)\|_{\mathcal{L}_{1}}\|\hat{\bar{\eta}}_{\tau}\|_{\mathcal{L}_{\infty}} \cdots \nonumber\\
        &+ \|k_g H(s)C(s)\|_{\mathcal{L}_{1}}\|r_{\tau}\|_{\mathcal{L}_{\infty}} + \| H(s)f(s)\|_{\mathcal{L}_{1}}+ \|x_{in_{\tau}}\|_{\mathcal{L}_{\infty}}
    \end{align}
Next, applying the triangular relationship for norms to the bound in \eqref{eq:bound}, with
% \begin{align}
%     |\| \hat{x}_{\tau}\|_{\mathcal{L}_{\infty}} -  \| x_{\tau}\|_{\mathcal{L}_{\infty}} |  \leq         \sqrt{ \frac{W_{\max}}{\lambda_{\min}(P)\Gamma_1} + \frac{\zeta_{\max}}{\lambda_{\min}(P)\Gamma_2}}
% \end{align}
        the projection operators ensuring that the error parameters $\Tilde{W}$ and $\Tilde{\bar{\zeta}}$ are bounded,  we have $\|\hat{\Bar{\eta}}_{\tau}\|_{\mathcal{L}_{\infty}}\leq L_1 \| x_{\tau}\|_{\mathcal{L}_{\infty}}$. 
    %     Substituting for $\| x_{\tau}\|_{\mathcal{L}_{\infty}}$ yields
    % \begin{align}\label{eq:bound3}
    %     \|\hat{\Bar{\eta}}_{\tau}\|_{\mathcal{L}_{\infty}} \leq L_1 \left (  \| \hat{x}_{\tau}\|_{\mathcal{L}_{\infty}}  +    \sqrt{ \frac{W_{\max}}{\lambda_{\min}(P)\Gamma_1} + \frac{\zeta_{\max}}{\lambda_{\min}(P)\Gamma_2}}             \right )
    % \end{align}
    Then the bound on $\| \hat{x}_{\tau}\|_{\mathcal{L}_{\infty}}$ in \eqref{eq:prdict_tf}, with account of the stability condition in \eqref{eq:l1norm}, lead to
    \begin{align}
        &\|\hat{x}_{\tau} \|_{\mathcal{L}_{\infty}} \leq \cdots \nonumber\\
        &\frac{\lambda_1 \sqrt{ \frac{W_{\max}}{\lambda_{\min}(P)\Gamma_1} + \frac{\zeta_{\max}}{\lambda_{\min}(P)\Gamma_2}} + \|G(s)\|_{\mathcal{L}_{1}}\|\hat{\eta}_{\tau}\|_{\mathcal{L}_{\infty}}+\dots   }{1-\lambda_1} \nonumber \\
        &\frac{\|k_g H(s) C(s \|_{\mathcal{L}_{1}} \| r_{\tau} \|_{_{\mathcal{L}_{\infty}}} + \| H(s)f(s)\|_{\mathcal{L}_{1}}+ \|x_{in_{\tau}} \|_{_{\mathcal{L}_{\infty}}}}{1-\lambda_1}
    \end{align}
    Since the bound on the right hand side is uniform, $\hat{x}(t)$ is uniformly bounded. Application of Barbalat's lemma leads to the asymptotic result $\underset{t \rightarrow \infty}{\lim}\Tilde{x}(t)=0$. Note that $\hat{\eta}_{\tau}$ is bounded because $\Tilde{x}_{\tau}$ is shown to be bounded from Lemma \ref{lem:pred_er} and $\eta(s)$ is bounded due to $\Delta(x) \subset D_x$.
    
    
    \end{proof}
Next, we present the main result of this paper in Theorem \ref{thrm:1}, which provides the proof of convergence of $x$ to $x_{ref}$ and $u$ to $u_{ref}$.
    \begin{theorem} \label{thrm:1}
    For 
    % the system in \eqref{eq:er_gnrl_st_sp} and the controller defined in \eqref{eq:totl_contrl_law} with the state predictor dynamics given by \eqref{eq:st_prdctr} and 
    the adaptive control law in \eqref{eq:u_ad_tf}, subject to the $\mathcal{L}_1$-norm condition in \eqref{eq:l1norm}, we have
    \noindent\begin{minipage}{0.5\linewidth}
\begin{equation}
 \|x_{ref} - x\|_{\mathcal{L}_{\infty}} \leq \gamma_1 \label{eq:v1}
\end{equation}
\end{minipage}%
\begin{minipage}{0.5\linewidth}
\begin{equation}
  \|u_{ref} - u\|_{\mathcal{L}_{\infty}} \leq \gamma_2 \label{eq:v2}
\end{equation}
\end{minipage}\par\vspace{\belowdisplayskip}
\noindent\begin{minipage}{0.5\linewidth}
\begin{equation}
\displaystyle  \lim_{t\rightarrow \infty} \|x_{ref}(t) - x(t)\|_{\mathcal{L}_{\infty}} = 0 \label{eq:Ld1}
\end{equation}
\end{minipage}%
\begin{minipage}{0.5\linewidth}
\begin{equation}
\displaystyle  \lim_{t\rightarrow \infty} \|u_{ref}(t) - u(t)\|_{\mathcal{L}_{\infty}} = 0 \label{eq:L_s=Ld+Ld'/2} 
\end{equation}
\end{minipage}\par\vspace{\belowdisplayskip}
where $\gamma_1$ and $\gamma_2$ are derived in \eqref{eq:gamma_1} and \eqref{eq:gamma_2}, respectively.
    \end{theorem}
    \begin{proof}
    The response of the closed-loop system in \eqref{eq:er_unct} with the \ladap~in \eqref{eq:u_ad_tf} can be written in the frequency domain as
%     \begin{align}
%         x(s) &= G(s)\Delta(x(s)) + G(s)\zeta^T x(s) + k_g H(s)C(s)r(s) \cdots \nonumber\\
%         &+ \scriptstyle H_1(s) f(s)-   H(s)C(s)(\Tilde{\eta}(s) + \Tilde{\Bar{\eta}}(s) +  \epsilon_1(x(s)))+ x_{in}(s)
%     \end{align}
%     the close-loop reference system is then
%       \begin{align}
%       x_{ref}(s) &= H(s)k_g C(s)r(s)+ G(s)\zeta^T x_{ref}(s) + x_{in}(s) \dots \nonumber \\
% &+ H_1(s) f(s) + G(s)\Delta(x_{ref}(s))
%     \end{align}
%     then we have 
%     \begin{align}\label{eq:ref_er}
%       x_{ref}(s)-x(s)  &= G(s)\zeta^T (x_{ref}(s) - x(s)) \dots \nonumber \\
%        &+ G(s)(\Delta(x_{ref}(s))-\Delta(x(s))) + C(s)\Tilde{x}(s)
%     \end{align}
%     which implies that
     \begin{align}
      &\|(x_{ref}-x)_{\tau} \|_{\mathcal{L}_{\infty}} \leq \|G(s)\zeta^T \|_{\mathcal{L}_{1}} \|(x_{ref}(s) - x(s))_{\tau} \|_{\mathcal{L}_{\infty}}\scriptstyle \dots \nonumber \\
       &+ \|C(s)\|_{\mathcal{L}_{1}}\|\Tilde{x}_{\tau}\|_{\mathcal{L}_{\infty}} + \|G(s)\|_{\mathcal{L}_{1}}\|(\Delta(x_{ref})-\Delta(x))_{\tau}\|_{\mathcal{L}_{\infty}}
    \end{align}
    Then the bound in \eqref{eq:bound} lead to the uniform upper bound
      \begin{align}\label{eq:gamma_1}
      &\|(x_{ref}-x)_{\tau} \|_{\mathcal{L}_{\infty}} \leq \dots  \nonumber \\
      % \frac{\|C(s)\|_{\mathcal{L}_{1}}}{1-\|G(s) \|_{\mathcal{L}_{1}}L_1}\|\Tilde{x}_{\tau}\|_{\mathcal{L}_{\infty}}\dots \nonumber \\
      %  & + \frac{\|G(s)\|_{\mathcal{L}_{1}}}{1-\|G(s) \|_{\mathcal{L}_{1}}L_1}\|(\Delta(x_{ref})-\Delta(x))_{\tau}\|_{\mathcal{L}_{\infty}}\dots \nonumber \\
       &   \gamma_1 = \frac{\|C(s)\|_{\mathcal{L}_{1}}}{1-\|G(s) \|_{\mathcal{L}_{1}}L_1} \sqrt{ \frac{W_{\max}}{\lambda_{\min}(P)\Gamma_1} + \frac{\zeta_{\max}}{\lambda_{\min}(P)\Gamma_2}} \dots \nonumber \\
       & + \frac{\|G(s)\|_{\mathcal{L}_{1}}}{1-\|G(s) \|_{\mathcal{L}_{1}}L_1}\|(\Delta(x_{ref})-\Delta(x))_{\tau}\|_{\mathcal{L}_{\infty}} 
    \end{align}
  Note that by invoking the idea of \textit{projection} operator we can claim boundedness on the term $\|(\Delta(x_{ref})-\Delta(x))_{\tau}\|_{\mathcal{L}_{\infty}}$. Further, using Lemma \ref{lem:conv}, with Assumption \ref{asum:1}, we can say that as $\Tilde{x}(t)\rightarrow 0$, $\Delta(x)\rightarrow \Delta(x_{ref})$.
  
  Now, from \eqref{eq:ref_er}, we have 
    \begin{align}\label{eq:ref_er}
      x_{ref}&(s)-x(s)  = (\mathbb{I}-G(s)\zeta^T)^{-1} C(s)\Tilde{x}(s) \dots \nonumber \\
       &+ (\mathbb{I}-G(s)\zeta^T)^{-1} G(s)(\Delta(x_{ref}(s))-\Delta(x(s))) 
    \end{align}
    Therefore, from \textit{final value theorem} and Lemma \ref{lem:conv}, we know that $ \lim_{s\rightarrow0} s \Tilde{x}(s) =  \lim_{t\rightarrow \infty}  \Tilde{x}(t) =0$.
    % \begin{align}
    %     \lim_{s\rightarrow0} s \Tilde{x}(s) =  \lim_{t\rightarrow \infty}  \Tilde{x}(t) =0
    % \end{align}
    Then, since the reference system is BIBO and $(\mathbb{I}-G(s)\zeta^T)^{-1}$ is stable, with invoking the \textit{finite value theorem} and the limit of $\Tilde{x}(t)$ from above, it leads to 
    
    \begin{align}
        &\lim_{t\rightarrow \infty} (x_{ref}(t) - x(t))= \lim_{s \rightarrow 0} s (x_{ref}(s)-x(s))=0 
       % & = \lim_{s \rightarrow 0} s (\mathbb{I}-G(s)\zeta^T)^{-1} C(s)\Tilde{x}(s) \dots \nonumber\\
       % &+ \lim_{s \rightarrow 0} s (\mathbb{I}-G(s)\zeta^T)^{-1} G(s)(\Delta(x_{ref}(s))-\Delta(x(s)))\nonumber \\
        %  & = \lim_{s \rightarrow 0}  (\mathbb{I}-G(s)\zeta^T)^{-1} C(s)(s\Tilde{x}(s)) \dots \nonumber\\
        % &+ \lim_{s \rightarrow 0}  (\mathbb{I}-G(s)\zeta^T)^{-1} G(s)s(\Delta(x_{ref}(s))-\Delta(x(s)))\nonumber \\
        % &=0
    \end{align}
    which leads to \eqref{eq:Ld1}.  
    Next, we will derive the second bound in \eqref{eq:v2}, for which, by using Lemma \ref{lem:conv} with Assumption \ref{asum:1}, we have 
    % \begin{align}\label{eq:law_er}
    %    & u_{ref}(s) - u(s) = -(C(s) \bar{\zeta}^T+ k_m^T) (x_{ref}(s)-x(s)) \dots \nonumber \\
    %    &+C(s)\Tilde{\Bar{\eta}}(s)-C(s)(\Delta(x_{ref}(s))-\Delta(x(s)))
    % %   &-C(s)( \bar{\zeta}^T+ k_m^T) (x_{ref}(s)-x(s)
    %     % &  - C(s)(\hat{\eta}(s) + \hat{\Bar{\eta}}(s)- k_g r(s)) 
    % \end{align}
    % which, again by using Lemma \ref{lem:conv} with Assumption \ref{asum:1}, simplifies to 
    % \begin{align}
    %    & u_{ref}(s) - u(s) = -(C(s) \bar{\zeta}^T+ k_m^T) (x_{ref}(s)-x(s)) \dots \nonumber \\
    %    &+C(s)\Tilde{\Bar{\eta}}(s)
    % \end{align}
    % which implies 
    \begin{align}
       & u_{ref}(s) - u(s) = -(C(s) \bar{\zeta}^T+ k_m^T) (x_{ref}(s)-x(s)) \dots \nonumber \\
       &+C(s)(H(s)^{-1}\Tilde{x}(s)- \Tilde{\eta}(s)- \epsilon_1(x(s)))
    \end{align}
    and consequently, we have:
    \begin{align}\label{eq:gamma_2}
        & \|(u_{ref} - u)_{\tau}\|_{\mathcal{L}_{\infty}} \leq \gamma_2 = \|C(s)H(s)^{-1}\|_{\mathcal{L}_{1}}\|\Tilde{x}_{\tau}\|_{\mathcal{L}_{\infty}}\dots \nonumber \\
       &+\|(C(s) \bar{\zeta}^T+ k_m^T)\|_{\mathcal{L}_{1}} \|(x_{ref}-x)_{\tau}\|_{\mathcal{L}_{\infty}} \dots \nonumber \\
       % &+\|C(s)H(s)^{-1}\|_{\mathcal{L}_{1}}\|\Tilde{x}_{\tau}\|_{\mathcal{L}_{\infty}}\dots \nonumber \\
       &- \|C(s)\|_{\mathcal{L}_{1}}\|\Tilde{\eta}_{\tau}\|_{\mathcal{L}_{\infty}}- \|C(s)\|_{\mathcal{L}_{1}}\|\epsilon_1(x_{\tau}\|_{\mathcal{L}_{\infty}}
    \end{align}
    
    Hence, the above relation can be claimed to be bounded. For \eqref{eq:L_s=Ld+Ld'/2}, the boundedness and the uniform continuity of $\Tilde{x}(t)$ and $\Tilde{\bar{\eta}}(t)$ with the  application of Barbalat's lemma  imply that $\dot{\Tilde{x}}(t)$ is bounded and leads to $\lim_{t\rightarrow \infty}\dot{\Tilde{x}}(t)=0$. Consequently, $lim_{t\rightarrow \infty}\Tilde{\Bar{\eta}}(t)=0$. 
    % Then the limit in \eqref{eq:L_s=Ld+Ld'/2} follows immediately from \eqref{eq:law_er}  and \eqref{eq:v1}.
    
    
    \end{proof}
    
    
    % \subsection{$\mathcal{L}_1$ Adaptive Control Using Deep Nets}
%     Algorithm

% Insert Figure of framework

% The DNN in the adaptive controller is trained over training dataset $Z^M=\{x_i,\Delta'(x_i)\}$, where the $\Delta'(x_i)$ are D-MRGeN estimates of the uncertainty. The training dataset $Z^M$ is randomly drawn from a larger data buffer $\mathcal{B}$.
% Not every pair of data $\{x_i, \Delta'(x_i)\}$ from D-MRGeN is added to the training buffer $\mathcal{B}$. We qualify the input-target pair based on kernel independence test such that to ensure that we collect locally exciting independent information which provides a sufficiently rich representation of the operating domain. Since the state-uncertainty data is the realization of a Markov process, such a method for qualifying data to be sufficiently independent of previous data-points is necessary.

% \begin{remark}
%    Discuss Stability Analysis for Controller with DNN
% \end{remark}


     \subsection{Stability Analysis for Controller with DNN}
    % We here provide the stability guarantee for deep $\mathcal{L}_1$ adaptive control framework.
    The generalization error of a machine learning model is defined as the empirical loss of the training set minus the expected loss of test set $\hat{\Delta}(x) - f_{\theta}(x) \leq \epsilon_G$,
    % This property determines the ability of the trained model to generalize well from the learning data to new unseen data. The capability of the model to extrapolate from training data to new data is determined. The \textit{generalization} error is typically defined as
    % \begin{align}
    %     \hat{\Delta}(x) - f_{\theta}(x) \leq \epsilon_G
    % \end{align}
    where $f_{\theta}$ is the learned approximation to the model uncertainty. 
    % with parameters $\theta \in \Theta$, where $\Theta$ is the space of parameters, i.e. $f_{\theta}: \mathbb{R}^n \rightarrow \mathbb{R}^m$.
    Then, using \eqref{eq:totl_contrl_law} and using the system in \eqref{eq:er_gnrl_st_sp}, and by
    % we can re-write the system error dynamics as
    % \begin{align}\label{eq:er_dyn2}
    % \dot{\Tilde{x}} = A_m \Tilde{x} + B_1( f_{\theta}(x) - \Delta(x) + \Tilde{\Bar{\Delta}}(x))
    % \end{align}
    adding and subtracting the term $\Delta'(x)$ and using the training and generalization error definitions we can re-write the system error dynamics as
    \begin{align}\label{eq:er_dyn3}
    \dot{\Tilde{x}} = A_m \Tilde{x} + B_1( f_{\theta}(x)  -\Delta'(x)  + \Delta'(x) -\Delta(x) + \Tilde{\Bar{\Delta}}(x))
    \end{align}
     where the training error $(\Delta'(x)-\Delta(x))$ is assumed to be zero as also done in \cite{joshi2019deep}. The term $(f_{\theta}(x)  -\Delta'(x))$ is the generalization error of our machine learning model. Therefore, the final predictor error dynamics looks like  \begin{align}\label{eq:er_dyn4}
    \dot{\Tilde{x}} = A_m \Tilde{x} + B_1( \epsilon_G + \Tilde{\Bar{\Delta}}(x))
    \end{align}
    We then define a Lyapunov candidate function of the type 
    \begin{align}
        V(\Tilde{x},\Tilde{\Bar{\Delta}})=\Tilde{x}^T P \Tilde{x} + \frac{\Tilde{\Bar{\Delta}}^T \Tilde{\Bar{\Delta}}}{\Gamma_2}
    \end{align}
    Taking the time derivative of the above Lyapunov function we get $\dot{V}(\Tilde{x},\Tilde{\Bar{\Delta}})=-\Tilde{x}^T Q \Tilde{x} + 2 \epsilon_G B_1 P \Tilde{x} $,
    % \begin{align}
    %     \dot{V}(\Tilde{x},\Tilde{\Bar{\Delta}})=-\Tilde{x}^T Q \Tilde{x} + 2 \epsilon_G B_1 P \Tilde{x} 
    % \end{align}
    where $Q$ is the solution of Lyapunov equation $A_m^T P + P A_m= -Q$. To satisfy the condition $\dot{V}(\Tilde{x},\Tilde{\Bar{\Delta}})\leq 0$ we get the following upper bounds on the generalization error
    \begin{align}\label{eq:DNN_bound}
        \|\epsilon_G\|< \frac{\lambda_{\max}(Q)\|\Tilde{x}\|}{\lambda_{\min}(P)}
    \end{align}
    which implies that 
    for a generalization error lower than the bound in \eqref{eq:DNN_bound}, Lyapunov stability of \neural~is guaranteed.
    % \pmcomment{i) check if $\epsilon = \epsilon_G$ and if the derivative of V cancels out the $\Tilde{\bar{\Delta}}$ term? }

==> abstract-v2.tex <==


